Model reduction of port-Hamiltonian systems via neural networks

In this paper, we consider structure-preserving model reduction of port-Hamiltonian (pH) systems which extend classical Hamiltonian systems with dissipation and an input-output port. These pH systems are often used in multi-physics systems, as the interconnection of one or more \pH systems results again in a pH system. If particularly the system matrices associated with the interconnection and/or dissipation of a pH system are state-dependent, then the evaluation of standard reduced-order models (ROMs) may depend on the dimension of the original full-order model, resulting in high computational costs. To circumvent these high costs, we propose to use structure-preserving neural networks. In particular, we perform two steps: (1) we use the generalized manifold Galerkin projection to project the pH system onto the reduced space; then (2) we train a neural network to learn the map from the reduced-order state to the reduced-order interconnection and dissipation system matrices. To ensure that the resulting ROM is again a pH system, the architecture of the neural network is chosen such that the skew-symmetry and positive semi-definiteness of the reduced-order systems matrices are maintained. In a numerical example, we consider a nonlinear mass-spring-damper system with state-dependent system matrices. The numerical results show that the proposed method achieves a significant computational speed-up compared to the original \ROM with comparable accuracy.

==> Mymacros.tex <==


%Widetilde macros 
\newcommand{\newbmJ}{\widetilde{\bm{J}}}
\newcommand{\newbmR}{\widetilde{\bm{R}}}
\newcommand{\newbmQ}{\widetilde{\bm{Q}}}
\newcommand{\newbmB}{\widetilde{\bm{B}}}
\newcommand{\newfunch}{\widetilde{h}}

%Curl macros
\newcommand{\curlD}{\mathcal{D}}
\newcommand{\curlX}{\mathcal{X}}

%Bold macros
\newcommand{\bmA}{\bm{A}}
\newcommand{\bmj}{\bm{j}}
\newcommand{\bmc}{\bm{c}}
\newcommand{\bme}{\bm{e}}
\newcommand{\bmp}{\bm{p}}
\newcommand{\bmr}{\bm{r}}
\newcommand{\bmq}{\bm{q}}
\newcommand{\bmm}{\bm{m}}
\newcommand{\bmmu}{\bm{\mu}}
\newcommand{\bml}{\bm{l}}
\newcommand{\bmK}{\bm{K}}
\newcommand{\bmv}{\bm{v}}
\newcommand{\bmS}{\bm{S}}
\newcommand{\bmU}{\bm{U}}
\newcommand{\bmV}{\bm{V}}
\newcommand{\bmw}{\bm{w}}
\newcommand{\bmW}{\bm{W}}
\newcommand{\bmJ}{\bm{J}}
\newcommand{\bmR}{\bm{R}}
\newcommand{\bmP}{\bm{P}}
\newcommand{\bmB}{\bm{B}}
\newcommand{\bmD}{\bm{D}}
\newcommand{\bmH}{\bm{H}}
\newcommand{\bmE}{\bm{E}}
\newcommand{\bmM}{\bm{M}}
\newcommand{\bmL}{\bm{L}}
\newcommand{\bmQ}{\bm{Q}}
\newcommand{\bmX}{\bm{X}}
\newcommand{\bmY}{\bm{Y}}
\newcommand{\bmu}{\bm{u}}

% \R for the real domain and \C for the complex domain
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
%Natural number
\newcommand{\N}{\mathbb{N}}

%Macros for the state and output
\newcommand{\statex}{{\bm x}}
\newcommand{\statey}{{\bm y}}
\newcommand{\xapprox}{\tilde{\bm x}}
\newcommand{\xr}{\check{\bm x}}
\newcommand{\bmXr}{\check{\bmX}}
\newcommand{\yr}{\check{\bm y}}
\newcommand{\statexT}{\statex(t)}
\newcommand{\stateyT}{\statey(t)}
\newcommand{\xrT}{\xr(t)}
\newcommand{\yrT}{\yr(t)}

\newcommand{\ddt}{\frac{\rm d}{{\rm d} t}}
\newcommand{\xref}{\statex_{\rm ref}}

\newcommand{\ideN}{\mathbb{I}_{N}}
\newcommand{\ider}{\mathbb{I}_{r}}


% Macros for system matrices JRQBH
\newcommand{\Jr}{\check{\bmJ}}
\newcommand{\Rr}{\check{\bmR}}
\newcommand{\Hr}{\check{\bmH}}
\newcommand{\Br}{\check{\bmB}}
\newcommand{\Qr}{\check{\bmQ}}
\newcommand{\Jmat}[1]{\mathbf{J}_{#1}}%Notation for canonical Poisson matrices.
\newcommand{\jtwo}{\Jmat{2}}
\newcommand{\Jrnonl}{\check{\funcJ}_{{\rm nonl}}(\xr)}
\newcommand{\Rrnonl}{\check{\funcR}_{{\rm nonl}}(\xr)}
\newcommand{\Hrnonl}{\check{\mathcal{H}}_{{\rm nonl}}(\xr)}
\newcommand{\Brnonl}{\check{\mathcal{B}}_{{\rm nonl}}(\xr)}
\newcommand{\Hamlable}{\mathcal{H}}
\newcommand{\Hamlabler}{\check{\mathcal{H}}}
\newcommand{\DivHamFOM}{\nabla_{\statex}\Hamlable(\statex(t))}
\newcommand{\DivHamROM}{\nabla_{\xr}\Hamlable(\xr(t))}


%Macros for notations for the systems 
\newcommand{\SysLable}{\Sigma}
\newcommand{\SysLableLin}{\SysLable_{\rm Lin}}
\newcommand{\SigMSFOM}[1]{\SysLable_{\rm{MS},\rm{#1}}}
\newcommand{\SigMSROM}[1]{\hat{\SysLable}_{\rm{MS},\rm{#1}}}
\newcommand{\SigMSROMNew}[1]{\widetilde{\SysLable}_{\rm{MS},\rm{#1}}}
\newcommand{\IntSys}{{\rm int}}

% Notations for size
\newcommand{\snapsize}{nt}
\newcommand{\samplesize}{m}
\newcommand{\portsize}{m}
\newcommand{\FOMsize}{N}
\newcommand{\ROMsize}{r}
\newcommand{\DEIMsize}{d}
\newcommand{\nlsize}{r_n}
\newcommand{\freqsize}{p}
\newcommand{\PODFreSize}{M}

%Notations for special matrices 
\newcommand{\Vbar}{\overline{\bmV}}
\newcommand{\VmodiPOD}{\bmV_{\rm modi POD}}
\newcommand{\Vtilde}{\widetilde{\bmV}}

%Macros for functions
\newcommand{\EnergyFunc}{\mathbf{E}}
\newcommand{\Kryfunc}{{\rm kry}}
\newcommand{\real}{{\rm real}}
\newcommand{\dxdHfunc}{h}
\newcommand{\lossfunc}{\mathcal{L}}
\newcommand{\lossfuncFOM}{\widetilde{\mathcal{L}}}
\newcommand{\approxfunc}{\varphi}
\newcommand{\decfunc}{\eta}
\newcommand{\quadfunc}{\gamma}
\newcommand{\matset}{\mathbf{S}}
\newcommand{\matfunc}{\mathcal{F}}
\newcommand{\MatSetJR}{\mathbf{S}_{J,R}}
\newcommand{\MatFuncJR}{\mathcal{F}_{J,R}}
\newcommand{\funcD}{\mathcal{D}}
\newcommand{\funcE}{\mathcal{E}}
\newcommand{\funcV}{\mathcal{V}}
\newcommand{\funcW}{\mathcal{W}}
\newcommand{\funcJ}{\mathcal{J}}
\newcommand{\funcR}{\mathcal{R}}
\newcommand{\funcQ}{\mathcal{Q}}
\newcommand{\funcH}{\mathcal{H}}
\newcommand{\funcB}{\mathcal{B}}
\newcommand{\funcEr}{\check{\mathcal{E}}}
\newcommand{\funcJr}{\check{\mathcal{J}}}
\newcommand{\funcRr}{\check{\mathcal{R}}}
\newcommand{\funcQr}{\check{\mathcal{Q}}}
\newcommand{\funcHr}{\check{\mathcal{H}}}
\newcommand{\funcBr}{\check{\mathcal{B}}}
\newcommand{\residual}{{\bm r}}
\newcommand{\transfunc}{\mathcal{G}}
\newcommand{\transfuncr}{\check{\mathcal{G}}}

\newcommand{\ConFuncSet}{\bm{C}}

%Macros for ROBs
\newcommand{\VPOD}{\bmV_{\rm POD}}
\newcommand{\VPODforce}{\bmV_{\rm force}}
\newcommand{\VPODGMG}{\widetilde{\bmV_{\rm POD}}}
\newcommand{\VIRKA}{\bmV_{\rm IRKA}}


%Notation related to the DEIM
\newcommand{\DEIM}[1]{\ensuremath{\check{#1}}}
\newcommand{\DEIMsplitHam}{p}
\newcommand{\DEIMsplitfunc}{q}


%Macros related to the neural network
\newcommand{\decfuncNN}{\psi}
\newcommand{\NNparas}{\omega}


%Notation for the interconnected system
%\IntSys
%Notations for the motivating example with the MG projection
\newcommand{\MotiMGNota}[1]{\widetilde{#1}}
%Notations for the proof of the theorem that discuss the existence of the generalized matrix inverse
\newcommand{\Jcheck}{\check{\bmJ}}
\newcommand{\Rcheck}{\check{\bmR}}

%Command for the breakable algorithm
\makeatletter
\newenvironment{breakablealgorithm}
{% \begin{breakablealgorithm}
		\begin{center}
			\refstepcounter{algorithm}% New algorithm
			\hrule height.8pt depth0pt \kern2pt% \@fs@pre for \@fs@ruled
			\renewcommand{\caption}[2][\relax]{% Make a new \caption
				{\raggedright\textbf{\ALG@name~\thealgorithm} ##2\par}%
				\ifx\relax##1\relax % #1 is \relax
				\addcontentsline{loa}{algorithm}{\protect\numberline{\thealgorithm}##2}%
				\else % #1 is not \relax
				\addcontentsline{loa}{algorithm}{\protect\numberline{\thealgorithm}##1}%
				\fi
				\kern2pt\hrule\kern2pt
			}
		}{% \end{breakablealgorithm}
		\kern2pt\hrule\relax% \@fs@post for \@fs@ruled
	\end{center}
}
\makeatother

% abbreviations
\newcommand{\pH}{\textsf{pH}\xspace}
\newcommand{\NN}{\textsf{NN}\xspace}
\newcommand{\GMGProject}{\textsf{GMG}\xspace}
\newcommand{\LTRB}{\textsf{LT-RB}\xspace} %Reduced-order-basis based on the Laplace transformation
\newcommand{\QM}{\textsf{QM}\xspace} %Represents the quadratic manifold 
\newcommand{\DEIMAbb}{\textsf{DEIM}\xspace}
\newcommand{\DEIMAbbs}{\textsf{DEIMs}\xspace}
%\newcommand{\DEIM}{\textsf{DEIM}\xspace}
\newcommand{\IRKA}{\textsf{IRKA}\xspace}
\newcommand{\POD}{\textsf{POD}\xspace}
\newcommand{\FOM}{\textsf{FOM}\xspace}
\newcommand{\ROM}{\textsf{ROM}\xspace}
\newcommand{\FOMs}{\textsf{FOM}s\xspace}
\newcommand{\ROMs}{\textsf{ROM}s\xspace}
\newcommand{\MOR}{\textsf{MOR}\xspace}
\newcommand{\MORs}{\textsf{MOR}s\xspace}
\newcommand{\ROB}{\textsf{ROB}\xspace}
\newcommand{\ROBs}{\textsf{ROB}s\xspace}
\newcommand{\DAE}{\textsf{DAE}\xspace}
\newcommand{\DAEs}{\textsf{DAE}s\xspace}
\newcommand{\SP}{\textsf{SP}\xspace}
\newcommand{\SPG}{\textsf{SPG}\xspace}
\newcommand{\ES}{\textsf{ES}\xspace}
\newcommand{\IRPH}{\textsf{IRPH}\xspace}

 %Notations for manifolds (GMG)
 \newcommand{\ManiFOM}{\mathcal{M}}
\newcommand{\ManiROM}{\hat{\ManiFOM}}

\newcommand{\LineWidth}{1}
\newcommand{\MarkSize}{3}
\newcommand\tstrut{\rule{0pt}{2.4ex}}
\newcommand{\errorH}{e_{\Hamlable_2}}
\newcommand{\errorHinf}{e_{\Hamlable_{\infty}}}
\newcommand{\errorOutput}{e_{\statey}}
\newcommand{\errorState}{e_{\statex, {\rm recon}}}
\newcommand{\errorProj}{e_{\statex, {\rm proj}}}
\newcommand{\errorApp}{e_{\statex, {\rm app}}}
\newcommand{\errorEnergy}{e_{\rm energy}}
